Fractal Weyl law for the Ruelle spectrum of Anosov flows

On a closed manifold $M$, we consider a smooth vector field $X$ that generates an Anosov flow. Let $V\in C^{\infty}\left(M;\mathbb{R}\right)$ be a smooth function called potential. It is known that for any $C>0$, there exists some anisotropic Sobolev space $\mathcal{H}_{C}$ such that the operator $A=-X+V$ has intrinsic discrete spectrum on $\mathrm{Re}\left(z\right)>-C$ called Ruelle resonances. In this paper, we show a fractal Weyl law: the density of resonances is bounded by $O\left(\left\langle \omega\right\rangle ^{\frac{n}{1+\beta_{0}}}\right)$ where $\omega=\mathrm{Im}\left(z\right)$, $n=\mathrm{dim}M-1$ and $0<\beta_{0}\leq1$ is the H\"older exponent of the distribution $E_{u}\oplus E_{s}$ (strong stable and unstable). We also obtain some more precise results concerning the wave front set of the resonances and the invertibility of the transfer operator. Since the dynamical distributions $E_{u}$,$E_{s}$ are non smooth, we use some semi-classical analysis based on wave packet transform associated to an adapted metric $g$ on $T^{*}M$ and construct some specific anisotropic Sobolev spaces.

==> figure/default <==
#FIG 3.2  Produced by xfig version 3.2.5c
Landscape
Center
Metric
A4      
100.00
Single
-2
1200 2
5 1 0 1 0 7 50 -1 -1 0.000 0 0 1 0 -499.552 1965.125 -550 2135 -480 1789 -405 2115
	0 0 1.00 60.00 120.00
5 1 0 1 0 7 50 -1 -1 0.000 0 0 1 0 -202.500 2250.000 -360 2160 -225 2070 -45 2160
	0 0 1.00 60.00 120.00
5 1 0 1 0 7 50 -1 -1 0.000 0 0 1 0 202.500 2250.000 45 2160 180 2070 360 2160
	0 0 1.00 60.00 120.00
5 1 0 1 0 7 50 -1 -1 0.000 0 0 1 0 652.500 2250.000 495 2160 630 2070 810 2160
	0 0 1.00 60.00 120.00
1 3 0 1 0 0 50 -1 20 0.000 1 0.0000 -450 2250 23 23 -450 2250 -428 2245
1 3 0 1 0 0 50 -1 20 0.000 1 0.0000 0 2250 23 23 0 2250 22 2245
1 3 0 1 0 0 50 -1 20 0.000 1 0.0000 450 2250 23 23 450 2250 472 2245
1 3 0 1 0 0 50 -1 20 0.000 1 0.0000 900 2250 23 23 900 2250 922 2245
4 0 0 50 -1 0 12 0.0000 2 180 315 -585 2475 $0$\001
4 0 0 50 -1 0 12 0.0000 2 180 390 1125 2250 $...$\001
4 0 0 50 -1 0 12 0.0000 2 180 315 -45 2475 $1$\001
4 0 0 50 -1 0 12 0.0000 2 180 315 405 2475 $2$\001
4 0 0 50 -1 0 12 0.0000 2 180 315 810 2520 $3$\001

